Development and Realization of Validation Benchmarks

In the field of modeling, the word validation refers to simple comparisons between model outputs and experimental data. Usually, this comparison constitutes plotting the model results against data on the same axes to provide a visual assessment of agreement or lack thereof. However, there are a number of concerns with such naive comparisons. First, these comparisons tend to provide qualitative rather than quantitative assessments and are clearly insufficient for making decisions regarding model validity. Second, they often disregard or only partly account for existing uncertainties in the experimental observations or the model input parameters. Third, such comparisons can not reveal whether the model is appropriate for the intended purposes, as they mainly focus on the agreement in the observable quantities. These pitfalls give rise to the need for an uncertainty-aware framework that includes a validation metric. This metric shall provide a measure for comparison of the system response quantities of an experiment with the ones from a computational model, while accounting for uncertainties in both. To address this need, we have developed a statistical framework that incorporates a probabilistic modeling technique using a fully Bayesian approach. A Bayesian perspective yields an optimal bias-variance trade-off against the experimental data and provide an integrative metric for model validation that incorporates parameter and conceptual uncertainty. Additionally, to accelerate the analysis for computationally demanding flow and transport models in porous media, the framework is equipped with a model reduction technique, namely Bayesian Sparse Polynomial Chaos Expansion. We demonstrate the capabilities of the aforementioned Bayesian validation framework by applying it to an application for validation as well as uncertainty quantification of fluid flow in fractured porous media.

==> TEXs/statement.tex <==
\newpage
\thispagestyle{empty}

\vspace*{\fill}
%use the English or the German version according to the language used in your thesis.

I hereby certify that I have prepared this thesis independently, and that only
those sources, aids, and advisers that are duly noted herein have been used
and/or consulted.

I further agree that this thesis is made accessible for scientific purposes by the 
library of the Institute for Modelling Hydraulic and Environmental Systems of 
the University of Stuttgart (Publication according to {\S}6 Abs. 1 UrhG). 
I agree that contents may be cited according to {\S}52 UrhG.\\[1cm]
Stuttgart, DATE\\[2cm]
FirstName LastName 


Hiermit erkl\"are ich, dass die vorliegende Arbeit von mir selbst und ohne fremde Hilfe,
lediglich unter Benutzung der hier aufgef\"uhrten Literatur, angefertigt worden ist. 
Diese Arbeit wurde in gleicher oder \"ahnlicher Form noch keiner anderen Pr\"ufungsbeh\"orde vorgelegt.

Ich stimme außerdem zu, dass die vorliegende Arbeit zu wissenschaftlichen Zwecken in den 
Bibliotheken des Instituts f\"ur Wasser- und Umweltsystemmodellierung der Universit\"at Stuttgart 
aufgestellt und zug\"anglich gemacht wird (Ver\"offentlichung nach {\S}6 Abs. 1 UrhG) und hieraus 
im Rahmen des {\S}52 UrhG zitiert werden kann.\\[1cm]
Stuttgart, DATE\\[2cm]
FirstName LastName

\endinput

==> TEXs/tipsandtricks.tex <==
\chapter{Tips And Tricks}
\thispagestyle{empty}

\newcommand{\examplecommand}[1]{\textbackslash\texttt{#1}}
\newcommand{\examplespace}[1]{\hspace{2cm}}

\section{Bibliography and citing}
\paragraph*{Bibliography:} For managing your bibliography, we recommend to use programs like:
\begin{itemize}
  \item \texttt{jabref}
  \item Mendeley
\end{itemize}
Use \examplecommand{cite}\{BibTexLabel\} when you refer to literature, like \cite{Bear1988,Flemisch2011}.
\paragraph*{Citing:} Check your given reference thoroughly! This does not only
mean text references or quotes, but also personal communication, input for
discussion/hypotheses/conclusions, ... .\\
Figures should also be emphasized
here: give references/sources to figures if you have copied or redraw them. Best would
be to even ask for the authors allowance.

\section{General Tips for Writing}
\begin{itemize}
  \item for non-running indices, like w for water are non-italic, use \examplecommand{textrm}\{w\}
        which produces $S_\textrm{w}$ instead of $S_w$.
  \item use the \examplecommand{DuMuX} command to get DuMuX written that way: \DuMuX
  \item for tables and figures use \examplecommand{caption}[ShortText]\{LongText\}
        then ShortText will appear in the list of figures/tables
        and LongText will appear directly below the figure/table
  \item fractions inside text look nicer with the \examplecommand{nicefrac}\{a\}\{b\}
        command \nicefrac{a}{b}
\end{itemize}

\section{Tables, Figures, and Equations}
This section provides some basic examples for tables, figures, and equations.
Table~\ref{tab:exampleTable} shows an exemplary table. 

\begin{table}
% table caption is above the table
\caption{This is an exemplary caption for your table. Table captions are above the actual table.}
\label{tab:exampleTable}       % Give a unique label
\centering
\begin{tabular}{lll}
\hline\noalign{\smallskip}
first & second & third  \\ % these are the column headers
\noalign{\smallskip}\hline\noalign{\smallskip}
number & number & number \\
number & number & number \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}

Figure~\ref{fig:exampleFigure} is an exemplary figure. 
Always reference your tables and figures at least once in the text. 
For normal figures, a width of approximately 0.8-0.9 of the text width \examplecommand{textwidth} is a good choice.
Be sure that the font size in plots is readable, which means at least the size of \examplecommand{tiny}. 
Every good plot should have at least axis labels and legend and may have a title if necessary.
Make sure that the lines, markers, and colors in your plots are easily visible, consistent through different figures,
meaningful, and distinguishable even for black and white print.

\begin{figure}
\centering
%for .eps, .png, etc use:
\includegraphics[width=0.2\textwidth]{\Pics/Logo_LH2_sw}
%for tikz figures use:
%\input{your_file.tex}
\caption{This is an exemplary caption for your figure. Figure captions are below the actual figure.}
\label{fig:exampleFigure}       % Give a unique label
\end{figure}

Equation~\eqref{eq:massBalance} is an example of a mass balance equation including components
for a multi-phase flow case.
Introduce every new variable in the vicinity of its first appearance. 
Be consistent in the format of the indices, sub- and superscripts and always label equations.

\begin{equation}\label{eq:massBalance} % Give a unique label
 \sum_{\alpha} \left[\frac{\partial}{\partial t}\left(\phi \rho_\alpha x^\kappa_\alpha S_\alpha \right) 
 + \nabla\cdotp \left(\rho_\alpha x^\kappa_\alpha \mathbf{v}_\alpha \right) 
 - \nabla\cdotp \left(\rho_\alpha \mathbf{D}_\mathrm{pm,\alpha} \nabla x^\kappa_\alpha \right) \right]= q^\kappa
 %\:\alpha \in \mathrm{n,w}
\end{equation}  


\section{Further Information}
\begin{enumerate}
  \item A thesis guideline is available at the homepage of Faculty 2:\\
        \href{http://www.f02.uni-stuttgart.de/studium/}{www.f02.uni-stuttgart.de/studium/}
  \item Good answer to many questions regarding LaTeX can be found in the web.
\end{enumerate}

\section{Additional Packages}
\subsection{Units}
This requires the \texttt{units} package. It is helpful to get the right
format for number, text and spacing. It works in both, math and text mode:\\
\examplecommand{unit}[1]\{m\} \hfill $\unit[1]{m}$\\
\examplecommand{unitfrac}[1]\{m\}\{s\} \hfill \unitfrac[1]{m}{s}\\

\subsection{Todonote}
This requires the \texttt{todonote}
\todo{With this package nice todos can be created}{package.}\\
You can even use them inline:
\todo[inline]{This is an inline todo note}


\endinput

